The structure of branching in Anosov flows of 3-manifolds

In this article we study the topological structure of the lifts to the universal of the stable and unstable foliations of $3$-dimensional Anosov flows. In particular we consider the case when these foliations do not have Hausdorff leaf space. We completely determine the structure of the set of non separated leaves from a given leaf in one of these foliations. As a consequence of this suspensions are characterized, up to topological conjugacy, as the only $3$-dimensional Anosov flows without freely homotopic closed orbits. Furthermore the structure of branching is related to the topology of the manifold: if there are infinitely many leaves not separated from each other, then there is an incompressible torus transverse to the flow. Transitivity is not assumed for these results. Finally, if the manifold has negatively curved fundamental group we derive some important properties of the limit sets of leaves in the universal cover.

==> mac.tex <==
% Adapted from gt3m book macros.
%
\def\Empty{}
%
% FLoat placement parameters:
%
\def\bottomfraction{.7}
\def\textfraction{0}
\def\floatpagefraction{.7}
%
% Definitions that use @ : 
\catcode`\@=11
% Redefine section heading to get smaller letters (this
% is copied from the original in rep12.sty)

\def\section{\@startsection {section}{1}{\z@}{-3.5ex plus -1ex minus 
-.2ex}{2.3ex plus .2ex}{\large\bf}}

% Here is \eqalign from plain TEX, resurrected here because latex
% refuses to make it easy to put equation numbers BETWEEN two 
% equations...
\def\eqalign#1{\,\vcenter{\openup\jot\m@th
  \ialign{\strut\hfil$\displaystyle{##}$&$\displaystyle{{}##}$\hfil
	\crcr#1\crcr}}\,}

% Modified description environment with paragraph indentation
% (lifted from report.sty)
\def\mydesc{\list{}{\labelwidth\z@ \itemindent-\leftmargin
\listparindent 1.5em
\let\makelabel\descriptionlabel}}
\let\endmydesc\endlist

% Matrix with smaller entries, modified from \matrix in plain.tex.
\def\Smatrix#1{\,\vcenter{\normalbaselines\baselineskip=2pt\m@th
    \ialign{\hfil$\scriptstyle ##$\hfil&&\hfil$\scriptstyle ##$\hfil\crcr
      \crcr
      #1\crcr\crcr}}\,}

% Our own caption style --

\def\fnum@figure{{\small Figure \thefigure}}
\def\fakefigure{\def\@captype{figure}}

\long\def\@makecaption#1#2{
    \vskip 10pt 
    \def\FCap{#2} \def\NoCap{\ignorespaces}
    \ifx \FCap\NoCap
       \setbox\@tempboxa\hbox{#1}  % This is to avoid the damn colon.
      \else
       \setbox\@tempboxa\hbox{#1: \small \it #2}
    \fi
    \ifdim \wd\@tempboxa >\hsize   % IF longer than one line:
        \unhbox\@tempboxa\par      %   THEN set as ordinary paragraph.
      \else                        %   ELSE  center.
        \hbox to\hsize{\hfil\box\@tempboxa\hfil}  
    \fi}

% Our page heading style:
\pagestyle{headings}
\oddsidemargin 1in
\evensidemargin 1in
\textwidth 5in
%\def\@evenhead{\rm \thepage\hfil \leftmark}%        Left heading.
\def\@oddhead{\hbox{}\rightmark \hfil \rm\thepage}% Right heading.
%\def\chaptermark#1{\markboth {\sc {\ifnum \c@secnumdepth >\m@ne
%      \@chapapp\ \thechapter. \ \fi #1}}{}}%
\def\sectionmark#1{\markright {\sc{\ifnum \c@secnumdepth >\z@
      \S\thesection.\hskip 1em\relax \fi #1}}}
%\def\thebibliography#1{\chapter*{References\@mkboth
%{\sc References}{\sc References}}\list
% {[\arabic{enumi}]}{\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
%    \advance\leftmargin\labelsep
%    \usecounter{enumi}}
%    \def\newblock{\hskip .11em plus .33em minus -.07em}
%    \sloppy
%    \sfcode`\.=1000\relax}

\catcode`\@=12
%
% Macro to define a new chapter without printing the big chapter heading 
\def\fakechapter#1{
	\refstepcounter{chapter}
	\chaptermark{#1}}

\def\oplabel#1{
  \def\OpArg{#1} \ifx \OpArg\Empty {} \else
  	\label{#1}
  \fi}
% Here we define the numbering conventions for theorems, etc.
% They are all numbered together, consecutively in each section.
%
\newtheorem{theoremSt}{Theorem}[section]
\newtheorem{corollarySt}[theoremSt]{Corollary}
\newtheorem{propositionSt}[theoremSt]{Proposition}
\newtheorem{lemmaSt}[theoremSt]{Lemma}
\newtheorem{defineSt}[theoremSt]{Definition}
\newtheorem{exampleSt}[theoremSt]{Example}
\newtheorem{exerciseSt}[theoremSt]{Exercise}
%
\def\NextItem{\refstepcounter{theoremSt} \item[\thetheoremSt]}
% This macro allows us to define a bunch of similar theorem-environments
% with automatic labelling and extra features.
%
\def\MakeStEnv#1{
  \newenvironment{#1}[2]{
  \begin{#1St} \oplabel{##1}%
  \global\def\CrntSt{\thetheoremSt}%
  \def\Labl{##1}\ifx\Labl\Empty{} \else {\rm (\Labl)\,}\fi%
  {\rm ##2}%
}{ 
  \end{#1St} }
}
\MakeStEnv{theorem}
\MakeStEnv{corollary}
\MakeStEnv{proposition}
\MakeStEnv{lemma}
\MakeStEnv{define}
\MakeStEnv{example}

\newenvironment{exercise}[1]{
  \small
  \begin{quote}	% To get indentation
    \begin{exerciseSt} \oplabel{#1}
    \rm
}{
    \end{exerciseSt}
  \end{quote}
  \medbreak\noindent
}
	
\def\lref#1{\ref{#1} (#1)}% Prints label as well as number
%
%
\def\defineterm#1{{\it #1}}
%
% Make a blank figure of given size with label in center.
%	\blankfig{label}{# of inches}{caption}
%
\newlength{\saveu}
\def\blankspace#1#2{
  \setlength{\saveu}{#2in}
  \divide\saveu by 2
  \vskip\saveu
  \centerline {\small \mbox{}#1}
  \vskip\saveu
}

\long\def\placefig#1#2#3#4{
  \begin{figure}[#4]
    \blankspace{#1}{#2}
    \caption[#1]{#3}
    \oplabel{#1}
  \end{figure}}
\long\def\blankfig#1#2#3{
  \placefig{#1}{#2}{#3}{htbp}}
\long\def\herefig#1#2#3{
  \par\noindent\vbox{
  \blankspace{#1}{#2}
  \fakefigure\caption[#1]{#3}
  \oplabel{#1}
  \vspace{\intextsep}
  }}
\long\def\botfig#1#2#3{
  \placefig{#1}{#2}{#3}{b}}

% figure macros that insert actual postscript files:

\long\def\ifig#1#2#3#4#5{
  \begin{figure}[#5]
   {\vss\special{psfile=#4}}
    \blankspace{#1}{#2}
    \caption[#1]{#3}
    \oplabel{#1}
  \end{figure}}
\long\def\realfig#1#2#3#4{
  \ifig{#1}{#2}{#3}{#4}{htb}}

%\def\blankfig#1#2#3{
%  \begin{figure}[hbp]
%  \blankspace{#1}{#2}
%  \caption{\it #3}
%  \label{#1}
%  \end{figure}
%}
\newcommand{\EndBlFig}{}		% Does nothing
%
\def\Subheading#1{\refstepcounter{theoremSt}
  \medskip\noindent{\bf \thetheoremSt\quad #1} 
  \par\medskip}
\def\numbergen#1{\refstepcounter{theoremSt} 
	\thetheoremSt \oplabel{#1}}
%
% This environment shouldn't be nested. 
%
\newenvironment{proof}[1]{
  \def\PfArg{#1}
  \ifx\PfArg\Empty
  	\edef\PfArg{\CrntSt}  \fi
 \startproof{\PfArg}%
}{ 
  \finishproof{\PfArg}
}
%
\newcommand{\startproof}[1]{
  \medbreak\mbox{}
  {\it Proof of #1:}%
}
\newcommand{\finishproof}[1]{ 
  \def\FPArg{#1}
  \ifx\FPArg\Empty
  	\def\FPArg{\CrntSt}  \fi
  \smallbreak\noindent\makebox[\textwidth]{\hfill\fbox{\FPArg}}
  \medbreak\noindent
}
%
\newcommand{\TE}{\BlankTableend}
\newcommand{\TS}{\BlankTable}
\newcommand{\BlankTableend}{}
\newcommand{\BlankTable}{\par  TABLE GOES HERE \par}
\newcommand{\UL}{\it}
\newcommand{\numreg}[3]{}		%Does nothing
%
%  math macros:
%
\def\extendor{\raisebox{0ex}[0in][0in]{\rule{0.5pt}{4ex}}}

\newcommand{\degree}{^\circ}
\newcommand{\degrees}{^\circ}
\newcommand{\complexes}{{\bf C}}
\newcommand{\dihedral}{{\bf D}_}
\newcommand{\gozto}{\mapsto}
\newcommand{\hyperbolic}{{\bf H}}
\newcommand{\hy}{{\bf H}}
\newcommand{\id}{{\rm id}}
\newcommand{\integers}{{\bf Z}}
\newcommand{\supperp}{^\perp}
\newcommand{\reals}{{\bf R}}
\def\zeemod #1{{\bf Z}_{#1}}
\newcommand{\euclidean}{{\bf E}}
\newcommand{\Euclidean}{{\bf E}}
\def\omicron{\circ}

\def\C{\complexes}
\def\Z{\integers}
\def\R{\reals}
\def\E{\Euclidean}
\def\H{\hyperbolic}
\def\Cstar{{\bf C_\ast}}
\def\Rstar{{\bf R_\ast}}
\def\SD{{\cal D}}
\def\empset{\phi}

\def\RP#1{{\bf RP}^{#1}}
\def\PSL#1{{\rm PSL}_{#1}}
\def\PSLtil#1{\til{\rm PSL}_{#1}}
\def\PGL#1{{\rm PGL}_{#1}}
\def\SL#1{{\rm SL}_{#1}}
\def\GL#1{{\rm GL}_{#1}}
\def\CP#1{{\bf CP}^{#1}}
\def\SU#1{{\rm SU}(#1)}
\def\PSU#1{{\rm PSU}(#1)}
\def\SO#1{{\rm SO}(#1)}
\def\O#1{{\rm O}(#1)}
\def\qi{{\bf i}}
\def\qj{{\bf j}}
\def\qk{{\bf k}}
\def\diff{\hbox{\it Diff\/}}

\def\Longmapsto{\longmapsto}    % Eventually this should be improved 
\def\bigrightarrow#1{\hbox to #1{\rightarrowfill}}
\def\bigleftarrow#1{\hbox to #1{\leftarrowfill}}
\def\iff{\Leftrightarrow}
\def\Iff{\Longleftrightarrow}
\def\implies{\Rightarrow}
\def\homeo{\cong}
\def\boundary{\partial}
\def\union{\cup}
\def\intersect{\cap}
\def\semidir{\mathrel{\hbox{\vrule depth-.03ex height1.1ex\kern-0.15em$\times$}}}
\def\isom{\hbox{isom}}
\def\nbd{{\cal N}}
\def\del{\nabla}
\def\til{\widetilde}
\def\length{{\rm length}}
\def\tr{{\rm tr}}
\def\empty{\phi}
\def\BSmatrix#1{
	\bigl[\Smatrix{#1}\bigr]
}
\def\Bmatrix#1{
	\left[\matrix{#1}\right]
}
% The small matrix that actually works:
\def\littlemat#1#2#3#4{
	{\bigl[ {#1 \atop #3} {#2 \atop #4} \bigr]}}
\def\littlevec#1#2{
	{\bigl[ {#1 \atop #2} \bigr]}}


==> serg.tex <==
% Definitions that use @ : 
\catcode`\@=11

% page heading on even pages gives chapter, but on same side of page
% as for odd pages. 


\newcommand{\ch}{\mbox{$\widehat{\bf C}$}}
\newcommand{\ii}{\mbox{${\cal I}$}}
\newcommand{\bp}{\mbox{$B^+$}}
\newcommand{\bn}{\mbox{$B^-$}}
\newcommand{\ag}{\mbox{${\cal A}_g$}}
\newcommand{\af}{\mbox{${\cal A}_f$}}
\newcommand{\hu}{\mbox{${\cal H}^u$}}
\newcommand{\et}{\mbox{$\eta _-$}}
\newcommand{\tsv}{\mbox{$\sigma ^s_e$}}
\newcommand{\hs}{\mbox{${\cal H}^s$}}
\newcommand{\hp}{\mbox{${\cal H}$}}
\newcommand{\tup}{\mbox{$\Theta ^u_+$}}
\newcommand{\tun}{\mbox{$\Theta ^u_-$}}
\newcommand{\tsp}{\mbox{$\Theta ^s_+$}}
\newcommand{\tsn}{\mbox{$\Theta ^s_-$}}
\newcommand{\vg}{\mbox{$\varphi_G$}}
\newcommand{\vf}{\mbox{$\varphi_F$}}
\newcommand{\vif}{\mbox{$\varphi^{\infty}_F$}}
\newcommand{\vig}{\mbox{$\varphi^{\infty}_G$}}
\newcommand{\vil}{\mbox{$\varphi^{\infty}_L$}}
\newcommand{\vi}{\mbox{$\varphi^{\infty}$}}
\newcommand{\vv}{\mbox{$\varphi _s$}}
\newcommand{\hlf}{\mbox{$X^L_F$}}
\newcommand{\hfl}{\mbox{$X^F_L$}}
\newcommand{\zf}{\mbox{$\zeta_F$}}
\newcommand{\zl}{\mbox{$\zeta_L$}}
\newcommand{\pin}{\mbox{$\partial _{\infty}$}}
\newcommand{\cc}{\mbox{$\cal C$}}
\newcommand{\ga}{\mbox{$\gamma $}}
\newcommand{\oo}{\mbox{$\cal O$}}
\newcommand{\ooo}{\mbox{$\cal J$}}
\newcommand{\ou}{\mbox{${\cal J}^u_+$}}
\newcommand{\rrr}{\mbox{$\times {\bf R}$}}
\newcommand{\rrrr}{\mbox{${\bf R}$}}
\newcommand{\rp}{\mbox{$[0,+\infty)$}}
\newcommand{\rr}{\mbox{$\times \{ 0 \}$}}
\newcommand{\pn}{\mbox{$\partial N$}}
\newcommand{\mi}{\mbox{$\widetilde M$}}
\newcommand{\ww}{\mbox{$\widetilde W$}}
\newcommand{\ti}{\mbox{$\partial \widetilde T$}}
\newcommand{\ttt}{\mbox{$\widetilde T$}}
\newcommand{\ppn}{\mbox{$\partial _+ N$}}
\newcommand{\lll}{\mbox{$l _{\epsilon}$}}
\newcommand{\iT}{\mbox{$i _{\widetilde T}$}}
\newcommand{\wwp}{\mbox{$\widetilde \Phi$}}
\newcommand{\w}{\mbox{$\widetilde {\partial _+ C}$}}
\newcommand{\pp}{\mbox{$\varphi$}}
\newcommand{\pw}{\mbox{$\varphi _{\widetilde T}$}}
\newcommand{\lmun}{\mbox{$\Gamma ^s \cup \Gamma ^u$}}
\newcommand{\gs}{\mbox{$\Gamma ^s$}}
\newcommand{\gu}{\mbox{$\Gamma ^u$}}
\newcommand{\ggs}{\mbox{${\cal F}^s_T$}}
\newcommand{\ggu}{\mbox{${\cal F}^u_T$}}
\newcommand{\gsr}{\mbox{$\Gamma ^s \times {\bf R}$}}
\newcommand{\gur}{\mbox{$\Gamma ^u \times {\bf R}$}}
\newcommand{\se}{\mbox{$S _{\epsilon}$}}
\newcommand{\gus}{\mbox{$\Gamma ^u \downarrow S_{\epsilon}$}}
\newcommand{\vt}{\mbox{$\overline \varphi _{\widetilde T}$}}
%\newcommand{\vv}{\mbox{$\varphi _{\widetilde T}$}}
\newcommand{\hh}{\mbox{${\bf H}^2$}}
\newcommand{\hhh}{\mbox{${\bf H}^3$}}
\newcommand{\lmS}{\mbox{$\Gamma ^s \downarrow S$}}
\newcommand{\lmU}{\mbox{$\Gamma ^u \downarrow S$}}
\newcommand{\lms}{\mbox{$\Gamma ^s \downarrow S_{\epsilon}$}}
\newcommand{\lmu}{\mbox{$\Gamma ^u \downarrow S_{\epsilon}$}}
\newcommand{\wall}{\mbox{$L \times \R$}}
\newcommand{\lap}{\mbox{$\Gamma ^s \cup \Gamma ^u \cup Q$}}
\newcommand{\tz}{\mbox{$\widetilde T \times \{ 0 \}$}}
\newcommand{\wt}{\mbox{$\widetilde T$}}
\newcommand{\wss}{\mbox{$\widetilde S$}}
\newcommand{\wn}{\mbox{$\widetilde N$}}
\newcommand{\si}{\mbox{$S^2_{\infty}$}}
\newcommand{\su}{\mbox{$S^1_{\infty}$}}
\newcommand{\sss}{\mbox{$S^s_{\infty}$}}
\newcommand{\sus}{\mbox{$S^u_{\infty}$}}
\newcommand{\s}{\mbox{$S ^1$}}
\newcommand{\fol}{\mbox{$\cal F$}}
\newcommand{\fn}{\mbox{$\cal \widetilde F$}}
\newcommand{\fs}{\mbox{${\cal F} ^s$}}
\newcommand{\fu}{\mbox{${\cal F} ^u$}}
\newcommand{\fss}{\mbox{${\cal F} ^{ss}$}}
\newcommand{\fuu}{\mbox{${\cal F} ^{uu}$}}
\newcommand{\fnss}{\mbox{$\widetilde {\cal F} ^{ss}$}}
\newcommand{\fnuu}{\mbox{$\widetilde {\cal F} ^{uu}$}}
\newcommand{\fns}{\mbox{${\widetilde {\cal F}}^s $}}
\newcommand{\fnu}{\mbox{${\widetilde {\cal F}}^u $}}
\newcommand{\fsS}{\mbox{${\cal F} ^s_S$}}
\newcommand{\fuS}{\mbox{${\cal F} ^u_S$}}
\newcommand{\fsT}{\mbox{${\cal F} ^s_T$}}
\newcommand{\fuT}{\mbox{${\cal F} ^u_T$}}
\newcommand{\fSS}{\mbox{$\widetilde{\cal F} ^s_{\cal S}$}}
\newcommand{\fUS}{\mbox{$\widetilde{\cal F} ^u_{\cal S}$}}
\newcommand{\fnuS}{\mbox{$\widetilde {{\cal F}}^u_S $}}
\newcommand{\fnsS}{\mbox{$\widetilde {{\cal F}}^s_S $}}
\newcommand{\ws}{\mbox{$\widetilde  W^s$}}
\newcommand{\wu}{\mbox{$\widetilde  W^u$}}
\newcommand{\hnt}{homotopically non trivial}
\newcommand{\up}{\mbox{${\cal U} _+$}}
\newcommand{\un}{\mbox{${\cal U} _-$}}
\newcommand{\Dp}{\mbox{$\Delta ^+$}}
\newcommand{\Dn}{\mbox{$\Delta ^-$}}
\newcommand{\fg}{\mbox{$\phi _g$}}
\newcommand{\h}{\mbox{$\bf H$}}

 

\def\@evenhead{\rm \leftmark \hfil \thepage}%        Left heading.
\def\chaptermark#1{\markboth {\sc {\ifnum \c@secnumdepth >\m@ne
      \@chapapp\ \thechapter. \ \fi #1}}{}}%

\catcode`\@=12


